Real-Time Differential Epidemic Analysis and Prediction for COVID-19 Pandemic

In this paper, we propose a new real-time differential virus transmission model, which can give more accurate and robust short-term predictions of COVID-19 transmitted infectious disease with benefits of near-term trend projection. Different from the existing Susceptible-Exposed-Infected-Removed (SEIR) based virus transmission models, which fits well for pandemic modeling with sufficient historical data, the new model, which is also SEIR based, uses short history data to find the trend of the changing disease dynamics for the infected, the dead and the recovered so that it can naturally accommodate the adaptive real-time changes of disease mitigation, business activity and social behavior of populations. As the parameters of the improved SEIR models are trained by short history window data for accurate trend prediction, our differential epidemic model, essentially are window-based time-varying SEIR model. Since SEIR model still is a physics-based disease transmission model, its near-term (like one month) projection can still be very instrumental for policy makers to guide their decision for disease mitigation and business activity policy change in a real-time. This is especially useful if the pandemic lasts more than one year with different phases across the world like 1918 flu pandemic. Numerical results on the recent COVID-19 data from China, Italy and US, California and New York states have been analyzed.

==> results_cases.tex <==
\section{Results and discussion}
\label{sec:results}

\subsection{Analysis for public data from China}

\begin{figure}[!ht]
  \centering
  \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRDP_hubei_IRD}\label{fig:SEIRDP_hubei_IRD}}
  \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRDP_hubei_BRN}\label{fig:SEIRDP_hubei_BRN}}
  \caption{(a)Predictions of the SEIRDP model and (b)Effective
    reproduction number for Hubei province, China  from January to middle April 2020\label{fig:Hubei_SEIRDP}}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.81\columnwidth]{SEIRDP_hubei_error}
\caption{The mean errors of the proposed SEIRDP model predictions for Hubei province, China.}
\label{fig:SEIRDP_hubei_error}
\end{figure}

We first show the modeling results for Hubei province of China from
earily Janaury to the middel of April, 2020.
Fig.~\ref{fig:Hubei_SEIRDP} (a) shows the time evoluation of the
numbers of the currently infected, the recovered and the death over
this period. Note that many public website shows the cumulative cases,
which is different than the currently infected, which the cumulative case
minus the reocvered and dead people. 

The cycles are the measured data, the solid line is the
last project in early April 2020 as China's pandemic outbreak has been
fully controlled. As we have all the historical data from early
outbreak to finish, the figure basically shows very good modeling
accuracy. Notice on Feb. 12, 2020, COVID-19 testing criteria has been
relaxed in Hubei Province, as a result, there is a huge jump of
confirmed infected cases, which can be viewed as outlier for the
date. As a result, the projection based on the history before Feb. 12
is a bit off the track of acutal cases. But for the most of time
points over the two month period, the projected and actual measured
cases match very well. TODO: present some error results.

Fig.~\ref{fig:Hubei_SEIRDP} (b) shows the effective reproduction
number, $R_t$, over the same period time. As we can see, $R_t$ become
leass than 1 around Feb. 19, which is about 3 weeks after city
lockdown in Wuhan on Feb 23, 2020. Feb. 19 is also close to the time
when the peak of infected people is reached as shown in
Fig.~\ref{fig:Hubei_SEIRDP} (a).  As a result, analysis and prediction
of effective reproduction number can give us more insights into how
the pandemic dynamics will play out and when the peak or turning
points will happen in the real time. Maybe we show see the day's death
rate figure (TODO).



% \begin{figure}[!ht]
%   \centering
%   \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRD_hubei_IRD}\label{fig:SEIRD_hubei_IRD}}
%   \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRD_hubei_BRN}\label{fig:SEIRD_hubei_BRN}}
%   \caption{(a)Predictions of the SEIRD model and (b)Effective reproduction number for Hubei province. 
%   \label{fig:Hubei_SEIRD}}
% \end{figure}

\subsection{Analysis and prediction for European and US data}

\begin{figure}[!ht]
  \centering
  \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRDP_Italy_IRD}\label{fig:SEIRDP_Italy_IRD}}
  \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRDP_Italy_BRN}\label{fig:SEIRDP_Italy_BRN}}
  \caption{(a) Predictions of the differential SEIRDP model and (b) Effective reproduction number for Italy from later Febrary to middle April 2020\label{fig:Italy_SEIRDP}}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.81\columnwidth]{SEIRDP_Italy_error}
\caption{The mean errors of the proposed SEIRDP model predictions for Italy.}
\label{fig:SEIRDP_Italy_error}
\end{figure}


Fig.~\ref{fig:Italy_SEIRDP} (a) shows COVID-19 disease modeling and
projection for Italy from late Feburary to midle of April 2020 as
Italy was mostly severely impacted by COVID-19 in Europe. As we can
see, our differential models match well for the historical data. The
prediction around early March is quite agressive as the actual growth
rate for both infected and deatth are very high. This is also
reflected in the effective reproduction numbers at those days as shown
in Fig.~\ref{ig:Italy_SEIRDP} (b). As of April 12, $R_r$ has reach to
around 2 and is still going downward. Based on our 10 day projection,
the currnetly infected cases will reach to the peak around April 17
with about 120K, with total accumulative cases about xxxK. 



% \begin{figure}[!ht]
%   \centering
%   \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRD_Italy_IRD}\label{fig:SEIRD_Italy_IRD}}
%   \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRD_Italy_BRN}\label{fig:SEIRD_Italy_BRN}}
%   \caption{(a)Predictions of the SEIRD model and (b)Effective reproduction number for Italy. 
%   \label{fig:Italy_SEIRD}}
% \end{figure}

For US data, we show the results for US, New York and California as
New York is the epic center of the COVID-19 in US. California has
largest population in US. The two states also have dramtically
transimission situations.  Fig.~\ref{fig:US_SEIRDP} (a) shows first
modeling and projection for Italy from late early March to midle of
April 2020 for the currently infected, recovery and death cases. The
results from the models match the given data very well.  

\begin{figure}[!ht]
  \centering
  \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRDP_US_IRD}\label{fig:SEIRDP_US_IRD}}
  \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRDP_US_BRN}\label{fig:SEIRDP_US_BRN}}
  \caption{(a) Predictions of the differential SEIRDP model and (b) Effective reproduction number for US from early March to middle April 2020\label{fig:US_SEIRDP}}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.81\columnwidth]{SEIRDP_US_error}
\caption{The mean errors of the proposed SEIRDP model predictions for US.}
\label{fig:SEIRDP_US_error}
\end{figure}



For California
The effective
repreduction number, $R_t$, shown in
Fig.~\ref{fig:SEIRDP_California_BRN} , which seems higher than basic
repreduction number, $R0$, which was estimated about 2-7 for
COVID-19~\cite{Liu:JTM'2020}, seems much higher. This may reflect
signficant portion of uncomfirmed and asymptotic population at the
beginning of this outbreaks in US (this is the cases for all the other
countries). But as time progresses, $R_t$ tends to level down to a
more reasonable range as more confirmed cases have been reported.

\begin{figure}[!ht]
  \centering
    \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRDP_California_BRN}\label{fig:SEIRDP_California_BRN}}
    \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRDP_California_error}\label{fig:SEIRDP_California_error}}
   \caption{ For California from from early Match to middle April
    2020 --  (a) The obtained effective reproduction number; (b) The mean errors
    of the proposed SEIRDP model predictions
    \label{fig:California_SEIRDP_data}}
\end{figure}

% \begin{figure}[!ht]
%   \centering
%   \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRD_US_IRD}\label{fig:SEIRD_US_IRD}}
%   \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRD_US_BRN}\label{fig:SEIRD_US_BRN}}
%   \caption{(a)Predictions of the SEIRD model and (b)Effective reproduction number for US. 
%   \label{fig:US_SEIRD}}
% \end{figure}

% \begin{figure}[!ht]
%   \centering
%   \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRDP_California_IRD}\label{fig:SEIRDP_California_IRD}}
%   \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRDP_California_BRN}\label{fig:SEIRDP_California_BRN}}
%   \caption{(a)Predictions of the SEIRDP model and (b)Effective reproduction number for California. 
%   \label{fig:California_SEIRDP}}
% \end{figure}

% \begin{figure}[!ht]
%   \centering
%   \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRD_California_IRD}\label{fig:SEIRD_California_IRD}}
%   \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRD_California_BRN}\label{fig:SEIRD_California_BRN}}
%   \caption{(a)Predictions of the SEIRD model and (b)Effective reproduction number for California. 
%   \label{fig:California_SEIRD}}
% \end{figure}

\begin{figure}[!ht]
  \centering
  \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRDP_NewYork_IRD}\label{fig:SEIRDP_NewYork_IRD}}
  \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRDP_NewYork_BRN}\label{fig:SEIRDP_NewYork_BRN}}
  \caption{(a) Predictions of the differential SEIRDP model and (b) Effective reproduction number for NewYork from early March to middle April 2020\label{fig:NewYork_SEIRDP}}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.81\columnwidth]{SEIRDP_NewYork_error}
\caption{The mean errors of the proposed SEIRDP model predictions for NewYork.}
\label{fig:SEIRDP_NewYork_error}
\end{figure}


% \begin{figure}[!ht]
%   \centering
%   \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRD_NewYork_IRD}\label{fig:SEIRD_NewYork_IRD}}
%   \subfigure[]{\includegraphics[width=0.49\linewidth]{SEIRD_NewYork_BRN}\label{fig:SEIRD_NewYork_BRN}}
%   \caption{(a)Predictions of the SEIRD model and (b)Effective reproduction number for NewYork. 
%   \label{fig:NewYork_SEIRD}}
% \end{figure}

